Synthesizing Switching Logic to Minimize Long-Run Cost

Given a multi-modal dynamical system, optimal switching logic synthesis involves generating the conditions for switching between the system modes such that the resulting hybrid system satisfies a quantitative specification. We formalize and solve the problem of optimal switching logic synthesis for quantitative specifications over long run behavior. Each trajectory of the system, and each state of the system, is associated with a cost. Our goal is to synthesize a system that minimizes this cost from each initial state. Our paper generalizes earlier work on synthesis for safety as safety specifications can be encoded as quantitative specifications. We present an approach for specifying quantitative measures using reward and penalty functions, and illustrate its effectiveness using several examples. We present an automated technique to synthesize switching logic for such quantitative measures. Our algorithm is based on reducing the synthesis problem to an unconstrained numerical optimization problem which can be solved by any off-the-shelf numerical optimization engines. We demonstrate the effectiveness of this approach with experimental results.

==> Makefile <==
# Makefile

# Set this to the basename of the .tex file
# This will also be the name of the generated .dvi, .ps and .pdf files
PAPER = quant-hscc

# Set this to the other source files that should be counted as 
# dependencies
OTHERSOURCES := quant-hscc.tex prob.tex prelim.tex single.tex
 
# Set this to the basenames of the files containing figures
# !!! If you do not want to regenerate the figures, run "make FIGURES="
FIGURES = 

.PHONY: ps
ps: $(PAPER).ps

.PHONY: pdf
pdf: $(PAPER).pdf


# run once, then re-run until it's happy
# input redirected from /dev/null is like hitting ^C at first error
$(PAPER).dvi: $(PAPER).tex $(OTHERSOURCES) $(FIGURES:%=%.eps)
	if latex $(PAPER).tex </dev/null; then \
		true; \
	else \
		stat=$$?; touch $(PAPER).dvi; exit $$stat; \
	fi
	bibtex $(PAPER)
	while grep "Rerun to get cross" $(PAPER).log; do \
		if latex $(PAPER).tex </dev/null; then \
			true; \
		else \
			stat=$$?; touch $(PAPER).dvi; exit $$stat; \
		fi; \
	done

$(PAPER).pdf: $(PAPER).dvi $(FIGURES:%=%.pdf) 
# Remove the .aux file because pdflatex wants it different
	rm -f $(PAPER).aux 
	if pdflatex $(PAPER).tex </dev/null; then \
		true; \
	else \
		stat=$$?; touch $(PAPER).pdf; exit $$stat; \
	fi
	bibtex $(PAPER)
	while grep "Rerun to get cross" $(PAPER).log; do \
		if pdflatex $(PAPER).tex </dev/null; then \
			true; \
		else \
			stat=$$?; touch $(PAPER).pdf; exit $$stat; \
		fi; \
	done

$(PAPER).ps: $(PAPER).dvi
	dvips -tletter -o $(PAPER).ps $(PAPER).dvi


clean:
	rm -f *.aux *.log *.ps *.dvi *.blg *.bbl *.toc *~ *.out *.tex1 *.tex2


# Generate PDF figures from the EPS ones
%.pdf: %.eps
	epstopdf $<



==> dcboost.tex <==
\subsection*{DC-DC Boost Converter}

In this case study, we synthesize switching logic for controlling
DC-DC boost converter circuits. The converter is presented as a
hybrid system with three modes of operation in Figure~\ref{fig:boost}.
The system remains in Mode 1 until the inductor current reaches the
reference current $I_{ref}$. The system remains in Mode 2 until
the inductor current becomes $0$. Then, the system switches to
Mode 3 where it remains till the output voltage remains over
the reference voltage $V_{ref}$. The inductor acquires and stores
the energy from the source in the first mode. In the second mode,
the stored energy is transferred to the capacitor and the load.
In the third mode, the excess energy of the capacitor is
transferred to the load. 

\begin{figure}[htpb]
\begin{center}
\scalebox{0.4}{\input{boost.pstex_t}}
\caption{DC-DC Boost Converter}
\label{fig:boost}
\end{center}
\end{figure}

The state space of the system is $X = \langle i_L \; u_C \rangle$.
The dynamics in the three modes is given by the state space
equation $\dot X = A_k X + B_k V$ where $k =1,2,3$ is the mode.
The coefficients of the equation are
\begin{verbatim}
to be texted

A1 = [(-rL-rs)/L 0; 0 -1/(C*(R+rC))];
B1 = [1/L; 0];

A2 = [(-rL-rd)/L -1/L; 
R/(R+rC)*(1/C - rC*(rL+rd)/L) -R/(R+rC)*(rC/L+1/(R*C))];
B2 = [1/L; R/(R+rC)*(rC/L)];

A3 = [0 0; 0 -1/((R+rC)*C)];
B3 = [0; 0];

\end{verbatim}

The control strategy is required to be resilient to load variations
so that the transient response is within some limits and the system
does not enter some unstable or chaotic region. Another requirement
is to keep the voltage ripple small. Both these requirements are
quantitative performance constraints. The traditional approach
described in several textbooks is pulsewidth modulation (PWM)
[CITEKassakian et al]. This approach is quite sensitive to
load variation. Gupta et al~[CITE Gupta-patra] propose a switching
scheme based on reference voltage and reference current for
controlling DC-DC boost converter circuits which addresses issues
of both small ripple and short transient response. We use our
technique to automatically discover the reference voltage and reference
current.

With $I_{ref} = 1.6$ and $V_{ref} = 12.05$, the behavior of the system
is presented in Figure~\ref{fig:boostplot1}.

\begin{figure}[htpb]
\begin{center}
\includegraphics[width=4in] {boost-plot1.eps}
\caption{DC-DC Boost Converter}
\label{fig:boostplot1}
\end{center}
\end{figure}



==> multi-old.tex <==
The approach presented in Section~\ref{sec-algo} 
can find the switching
states corresponding to optimal long-run behavior
{\em{for a given initial state}}. 
However, multimodal systems generally have more than one
initial state.

In this case, we use the approach of Section~\ref{sec-algo}
on each initial state and then define the optimal switching
guards as follows.  The guard
$\guard(\mode_i,\mode_j)$ for the transition from Mode $i$ to Mode $j$
contains 
$\state_k$ if
for some initial state, the optimal trajectory had
a jump from $\mode_i$ to $\mode_j$ at state $\state_k$.

\noop{
Let this procedure of
finding optimal switching states described in
Section~\ref{sec-algo} for a given 
single initial state $\hybridstate \in \init$ 
be called $getSS(\hybridstate)$
which returns the switching sequence
$\trajq = \mode_{i_1}, \mode_{i_2}, \ldots$ and switching states
$\switchlogic_{\hybridstate}$  containing $(\mode_i, \state_i) \in \guard_{\mode_i \mode_{j}}^{\mathit{over}}$ for each switch
$(\mode_i,\mode_{j}) $ in $\trajq$.
Algorithm~\ref{alg:multi} can be used 
to find optimal switching logic for a set of initial states.

\begin{algorithm}
%\SetLine
\KwIn{Set of initial state $\init$}
\KwOut{Switching Logic $\switchlogic$}

\ForEach{$(\mode_i,\mode_j) \in Q \times Q$}{
$\guard_{\mode_i \mode_j} = \{\}$ // Initialize guards to empty sets
}

\ForEach{$\hybridstate \in \init$}{
$(\trajq, \switchlogic_{\hybridstate}) = getSS(\hybridstate)$\;

\ForEach{switch $(\mode_i,\mode_j)$ in $\trajq$}{
$\guard_{\mode_i \mode_j} = \guard_{\mode_i \mode_j} \cup \{(\mode_i,\state_i)\} $ where $(\mode_i,\state_i) \in \switchlogic_{\hybridstate}$
}
}

return $\switchlogic = \{\guard_{\mode_i \mode_j}  | (\mode_i,\mode_j) \in Q \times Q \}$

\caption{Switching Logic Synthesis for Multiple Initial States}
\label{alg:multi}
\end{algorithm}
}

\noop{
The optimal trajectories are deterministic. 
We simply merge the guard states for each mode switch. 
This is correct because the hybrid
system formed by combining this synthesized switching logic
$\switchlogic$ is still deterministic and the trajectory
from each initial state is still of minimum cost. 
Using deterministic nature of the optimal trajectories,
}

The correctness of this approach for handling multiple
initial state relies on the
following \emph{non-interference} 
theorem. The proof is presented in the
full version~\cite{full}. %[EXT].

%We first make an important observations which provide the
%basis for extending our approach to multiple initial states.
%This is the \emph{non-interference} observation summarized
%in Theorem~\ref{thm-noninter} below.

\begin{theorem}
\label{thm-noninter}
From any two initial states, either the system enters a common
repetitive behavior $\traj_{rep}$ with minimum long-run
cost starting from both
initial states or their trajectories have no common state.
\end{theorem}

\noop{ 
It follows from the above theorem that two optimal trajectories 
starting from different initial states have a common
switching state only if both optimal trajectories have the
same repetitive behavior. Thus, any trajectory feasible 
from an initial state $\hybridstate \in \init$
in the hybrid system $\hs(\mds,\swl)$ formed using the switching logic
$\swl$ for the multimodal system $\mds$ has the same repetitive
behavior as the optimal trajectory from the initial state, and hence,
it is also of minimum cost.
Hence, all the trajectories in $\hs(\mds,\swl)$ are of minimum cost.
}

Nonlinear and hybrid systems show the phenomenon of
{\em bifurcation} and can have multiple equilibria and different
limit cycles from different initial states~\cite{sastry-book}.
The above algorithm enumerates over all initial states. So, it is
useful only when there are finite number of initial states. 
If the set of initial states is infinite, then we either sufficiently
sample the initial states and generate the guards by {\em{generalizing}}
the finitely many points we find on the optimal guards, or
consider a finite partition of the initial states. 

A common example of generalization is taking the convex hull 
of the points found.  This approach works whenever the human
designer can inform the synthesis algorithm about the 
{\em{form}} of the optimal guards.

\noop{
One special case, for example, is when optimal design satisfies
the following structure hypothesis.
% designer the 

\begin{definition}
For any two states, $(\mode, \state_1)$ and $(\mode, \state_2)$
some other state $(\mode, \state)$ is said to lie in the convex set of the two states, that is,   $(\mode, \state) \in \convex((\mode, \state_1),(\mode, \state_2))$ 
if and only if
for all variables $i$, 
$\state(i) = t \state_1(i) + (1-t) \state_2(i)$ for some $t\in[0,1]$.  
\end{definition}

\begin{definition}
\emph{Convex tube} property: Let $\switch_{ij}(\hybridstate)$ denote
the switching state from mode $i$ to $j$ in the trajectory 
starting at $\hybridstate$. The trajectories from a 
convex set of initial states are said to have the convex tube property
if they have a common mode switching sequence and
for any two trajectories starting from initial states
$(\mode_{\init}, \state_1)$ and $(\mode_{\init}, \state_2)$, and a third
trajectory starting from initial state 
$(\mode_{\init},\state) \in \convex((\mode_{\init}, \state_1),(\mode_{\init}, \state_2))$ 
$$ \switch_{ij}((\mode_{\init},\state)) \in \convex (\switch_{ij}((\mode_{\init},\state_1)),
\switch_{ij}((\mode_{\init},\state_2)))$$
for all mode switches $(i,j)$.
\end{definition} 
\begin{shypo}
The set of initial states can be partitioned into finite number of
convex subsets such that the optimal trajectories from each subset have
the \emph{convex tube} property. 
\end{shypo}

Now, if we are given this partition, synthesizing switching logic for a given
set of initial states can be done by enumerating over each of the convex
subsets. We compute the switching states for a finite set of initial states 
in the convex subset which span the entire subset. 
The switching set for the convex subset is the convex hull 
of these switching states. The final switching set is the union of the 
switching sets for each of the convex sets.  
}

%This extension is based on the observation made over the running
%example in Section~\ref{sec-alog}.

\subsubsection*{Running Example}
Given the set of initial states 
$16 \leq \thermoTemp \leq 26$ and $\thermoOut \in \{16,26\}$.
The set of initial states is partitioned into subsets where each
subset is a $0.1$ interval of room temperature $\thermoTemp$
and the outside temperature is $16$ or $26$. 
The guards discovered are: 
%\begin{eqnarray*}
$\;\guard_{HF} : \thermoTemp \geq 20.2 \wedge \thermoOut = 16, \;\;\;\; \guard_{FH} : \thermoTemp \leq  19.6 \wedge \thermoOut = 16, \;\;\;\;
\guard_{CF} : \thermoTemp \leq 20.0 \wedge \thermoOut = 26, \;\;\;\; \guard_{FC} : \thermoTemp \geq  20.3 \wedge \thermoOut = 26
$.
%\end{eqnarray*} 

%The key observation is that if the discovered optimal repetitive behavior for an initial state is reachable from any other initial state, then the optimal behavior from this initial state is also the same.


==> multirep.tex <==

TO MODIY TEXT BELOW / BIFURCATION OF NONLINEAR SYSTEMS





==> prelim.tex <==

\begin{definition}
A zeno trace is produced by an infinite sequence of mode switches during a bounded amount of time.
\end{definition}

\begin{theorem}
If the switching cost for modes is positive, that is, $s(\mode_i,\mode_j) > 0$ for all $i,j$, then any zeno trace is of infinite cost. 
\end{theorem}

\begin{proof}
Let the optimal synthesized automata have a zeno trace $\trace(\hybridstate)$ starting in the initial state $\hybridstate$.
Let the infinite switching start at time $t_1$ and switch $k$, that is, there are infinite number of switches between $t_1$ and $t_1 +\epsilon$. So, the cost of the trace is 
\begin{align*}
cost(\trace_{\hybridstate}) & \geq   
\displaystyle [\frac
{\int_{t}^{t+\epsilon} p(\state(t), \mode(t)) dt  }
{\int_{t}^{t+\epsilon} r(\state(t), \mode(t)) dt  } 
+ \displaystyle \lim_{l \rightarrow \infty} \frac {\displaystyle \sum_{i=k}^l s(\mode(t_i),\mode(t_{i+1}))} {\epsilon} \displaystyle ] \\
& \geq  \displaystyle \lim_{l \rightarrow \infty} \frac {\displaystyle \sum_{i=k}^l s(\mode(t_i),\mode(t_{i+1}))} {\epsilon} \rightarrow \infty
\end{align*}
So, any zeno trace has infinite cost if the mode switching cost is positive.
\end{proof}


\begin{theorem}
The mode-trace of any trajectory in a hybrid-system is either a finite sequence $$\mode(t_0), \mode(t_1), \ldots, \mode(t_k)$$ or is an infinite periodic sequence of the form $$\mode(t_1), \mode(t_2), \ldots, (\mode(t_l), \ldots, \mode(t_k))^*$$
\end{theorem}

\proof{
Sketch: Pigeon hole principle
}

We now introduce an important concept of dwell-time sequence which would be useful in presenting our approach to solve the optimum switching synthesis problem.

\begin{definition}
Dwell-time sequence:  We fix the sequence of modes to be $(1,2,\ldots,N)^*$. The dwell time-sequence $\dwellseq_{\hybridstate}$ of a trajectory $\trace_{\hybridstate}$ is sequence of time spent in different modes $$\{\dwelltime_{11},\dwelltime_{12},\ldots, \dwelltime_{1N},\ldots, \dwelltime_{j1}, \dwelltime_{j2}, \ldots, \dwelltime_{jk}, \ldots \dwelltime_{jN},\ldots \}$$ 
where $\dwelltime_{jk} \geq 0$ denotes the time spent in $j-th$ mode in the $k-th$ iteration over all the modes.  Let $NZ$ be a mapping that removes all the zero elements of the dwell time-sequence and 
$$NZ(\dwellseq_{\hybridstate}) = \{\dwelltime_{i_1j_1}, \dwelltime_{i_2j_2}, \ldots, \dwelltime_{i_k j_k}, \ldots \}$$ 
Given the dwell-time sequence $\dwellseq_{\hybridstate}$ and its non-zero mapping $NZ(\dwellseq_{\hybridstate})$ , the mode trajectory is given by
$$\trace^M_{\hybridstate}(t) = i_1 \;, \; 0 \leq t < \dwelltime_{i_1j_1}$$
$$\trace^M_{\hybridstate}(t) = i_k \;, \; \displaystyle \sum_{m=1}^{k-1} \dwelltime_{i_mj_m} \leq t <  \displaystyle \sum_{m=1}^{k} \dwelltime_{i_mj_m}$$
\end{definition}

\noop{We restrict our focus to hybrid systems which attain a \emph{stable behavior} after some finite time. 
It may be noted that the optimal synthesis problem is meaningful only when the system eventually reaches a stable behavior. }

Our approach requires the following to be provided by the user:
\begin{enumerate}
\item An over-approximation of the number of switches $K_S$ such that the system reaches \emph{stable behavior} in atmost $K_S$ mode switches. 
\item An over-approximation of the time taken $T_S$ such that the system reaches \emph{stable behavior} in atmost $T_S$ time units. 
\end{enumerate}


==> single.tex <==
 
We first consider the \emph{Optimal Switching Synthesis Problem} with a single initial state, that is, $I = \{(\state_0, \mode_0)\}$. 

\begin{algorithm}
%\SetLine
\KwIn{$MDS(X,Q)$, initial states $I$, initial over-approximation of the switching sets $S^{init}_{pq}$, over-approximation of the number of switches $K_S$ and time $T_S$}
\KwOut{Optimal Switching Logic $SL^{opt}$}
Compute $\dwellseq^{opt} = \argmin_{\dwellseq_{\hybridstate}} h(\dwellseq_{\hybridstate})$
Compute $NZ(\dwellseq_{\hybridstate}) = \{\dwelltime_{i_1j_1}, \dwelltime_{i_2j_2}, \ldots, \dwelltime_{i_k j_k}, \ldots \}$
$i_{k-1} = \trace^M_{\hybridstate}(t_{k-1})$
$i_k = \trace^M_{\hybridstate}(t_{k})$
$t_0 = 0, m = 1$
\ForEach{$\dwelltime_{i_mj_m}$ in $NZ(\dwellseq_{\hybridstate})$} {
$t_{m} = t_{m-1} + \dwelltime_{i_mj_m}$
}
\caption{Finding optimal switching logic $SL^{opt}$ with single initial state}
\label{alg:single}
\end{algorithm}

